Joint World Action Models through Differentiable Trajectory Optimization

Joint world action models (WAMs) generate future actions and states together, modeling world-action trajectories rather than actions alone. However, trajectory imitation does not ensure that these trajectories are task-effective or consistent with dynamics. We present world action trajectory optimization (WATO), which optimizes generated actions and future states jointly for control. WATO uses both as references in a dynamics-constrained trajectory optimization problem and differentiates the task loss through the optimized trajectory to train the generator. This makes generated trajectories task-aware and dynamics-consistent while using trajectory optimization only during training. At deployment, WATO directly generates candidate trajectories and ranks them with a world model, without iterative trajectory optimization. Across $7$ visual control environments, WATO improves average success from $79.9\%$ for the imitation joint WAM to $91.7\%$, outperforming strong model-based, goal-conditioned RL, and generative control baselines. Compared with cross-entropy method (CEM), WATO is on average $11.5\times$ faster and uses $600.5\times$ fewer world model evaluations at deployment.

==> fonts/inter-fonts.tex <==
% Local T1 metrics for the static Inter v4.1 faces. The 0.88 scale matches
% the sans-serif scale in the CoRe class; text and math retain their own faces.
\pdfmapfile{+fonts/inter.map}
\DeclareFontFamily{T1}{watointer}{}
\DeclareFontShape{T1}{watointer}{m}{n}{<-> s*[0.88] fonts/WATOInter-Regular}{}
\DeclareFontShape{T1}{watointer}{m}{it}{<-> s*[0.88] fonts/WATOInter-Italic}{}
\DeclareFontShape{T1}{watointer}{m}{sl}{<-> ssub*watointer/m/it}{}
\DeclareFontShape{T1}{watointer}{b}{n}{<-> s*[0.88] fonts/WATOInter-Bold}{}
\DeclareFontShape{T1}{watointer}{bx}{n}{<-> ssub*watointer/b/n}{}
\DeclareFontShape{T1}{watointer}{b}{it}{<-> ssub*watointer/b/n}{}
\DeclareFontShape{T1}{watointer}{bx}{it}{<-> ssub*watointer/b/n}{}
\DeclareFontFamily{T1}{watodisplay}{}
\DeclareFontShape{T1}{watodisplay}{b}{n}{<-> s*[0.88] fonts/WATOInterDisplay-Bold}{}
\newcommand{\watoDisplayBold}{\usefont{T1}{watodisplay}{b}{n}}
\renewcommand{\sfdefault}{watointer}
\DisableLigatures[f]{encoding=T1,family={watointer,watodisplay}}
\endinput

